Cryogenic Characterization of Low-Frequency Noise in 40-nm CMOS

This paper presents an extensive characterization of the low-frequency noise (LFN) at room temperature (RT) and cryogenic temperature (4.2 K) of 40-nm bulk-CMOS transistors. The noise is measured over a wide range of bias conditions and geometries to generate a comprehensive overview of LFN in this technology. While the RT results are in-line with the literature and the foundry models, the cryogenic behavior diverges in many aspects. These deviations include changes with respect to RT in magnitude and bias dependence that are conditional on transistor type and geometry, and even an additional systematic Lorentzian feature that is common among individual devices. Furthermore, we find the scaling of the average LFN with the area and its variability to be similar between RT and 4.2 K, with the cryogenic scaling reported systematically for the first time. The findings suggest that, as no consistent decrease of LFN at lower temperatures is observed while the white noise is reduced, the impact of LFN for precision analog design at cryogenic temperatures gains a more predominant role.

==> impact.tex <==
\section{Impact on analog design}
\label{section:impact}

- input-referred flicker stays roughly constant over bias - and to first order also in temperature \\
- very slight increase in input-referred noise \\

- thermal noise reducing (by a factor of about 2x) \\
-- shot noise \\
-- self-heating \\

- LFN mitigation in context of reduced thermal noise and slight increase in LFN very important \\
